Online Self-Attentive Gated RNNs for Real-Time Speaker Separation

Deep neural networks have recently shown great success in the task of blind source separation, both under monaural and binaural settings. Although these methods were shown to produce high-quality separations, they were mainly applied under offline settings, in which the model has access to the full input signal while separating the signal. In this study, we convert a non-causal state-of-the-art separation model into a causal and real-time model and evaluate its performance under both online and offline settings. We compare the performance of the proposed model to several baseline methods under anechoic, noisy, and noisy-reverberant recording conditions while exploring both monaural and binaural inputs and outputs. Our findings shed light on the relative difference between causal and non-causal models when performing separation. Our stateful implementation for online separation leads to a minor drop in performance compared to the offline model; 0.8dB for monaural inputs and 0.3dB for binaural inputs while reaching a real-time factor of 0.65. Samples can be found under the following link: https://kwanum.github.io/sagrnnc-stream-results/.

==> related.tex <==
% \section{Related Work}
% \label{sec:rel_work}

% Single channel speech separation is one of the fundamental problems in speech and audio processing. It was extensively explored over the years~\cite{logeshwari2012survey,martin2018single,ernst2018speech}, where traditionally signal processing techniques were applied to the task~\cite{choi2005blind}. Additionally, most previous research was conducted at the spectrum level of the input signal~\cite{wang2018supervised,ernst2018speech}. 

% Recently, deep learning models were suggested for the speech separation task, and have managed to vastly improve the performance over previous methods. \cite{hershey2016deep} suggests a clustering methods in which trained speech embeddings are being used for separation. \cite{yu2017permutation} proposed the Permutation Invariant Training (PIT) over the frame level for source separation, while~\cite{kolbaek2017multitalker} continue this line of work by suggesting the utterance level Permutation Invariant Training (uPIT). \cite{liu2019divide} suggest to use both PIT and clustering over the frame levels for speaker tracking. An excellent survey of deep learning based source separation methods was provided by~\cite{wang2018supervised}. A phase-sensitive objective function with an LSTM neural network was presented in \cite{erdogan2015phase}, showing an improvement of SDR over the CHiME-2 \cite{vincent2013second} dataset.


% \cite{wang2019deep} introduced a method to reconstruct the phase in the Fourier transform domain, by determined uniquely the absolute phase between two speakers based on their mixture signal. \cite{wang2018end} propose a novel method to separate speech signals in the time-frequency domain. The method use the magnitude and phase simultaneously in order to separate one speaker from the other. 

% An influential method was introduced by~\cite{luo2018tasnet}, where a deep learning method for speech separation over the time domain was presented. It employs thee components: an encoder, a separator and a decoder. Specifically they used a convolutional layer as the encoder, bidirectional LSTMs as the separator network, and a fully connected layer as the decoder that constructs the separated speech signals. Then,~\cite{luo2019conv} suggested to replace the separator network from LSTM to a fully convolutional model using block of time depth separable dilated convolution (Conv-Tasnet). \cite{zeghidour2020wavesplit} propose to infer a set of speaker representations via clustering to better separate the speakers.

% Recently, Conv-Tasnet was scaled by~\cite{zhang2020furcanext}, who proposed to train several separator networks in parallel to perform an ensemble. Dual Path RNN blocks were introduced by \cite{luo2019dual}. Such blocks, which we also use, first reorder the encoded representation and then process it across different dimensions. 

% Related to our goal of improving the performance on multiple speakers, \cite{takahashi2019recursive} introduce a recursive method for speaker separation, based on the Conv-Tasnet model. The authors suggested to separate out a single speaker at a time in a recursive manner. It is shown that a model that was trained to separate two and three speakers can separate four speakers. 

% Another line of work to note is studies which leverages speaker information during separation. In \cite{zmolikova2017speaker,delcroix2018single} a neural network employed estimated i-vectors~\cite{ivectors} in order to estimate masks, which extract the target speaker by generating beamformer filters, while \cite{wang2018voicefilter} proposed to use d-vectors~\cite{dvectors} as speaker embeddings and directly output the target separated sources. 

% A clustering method for speech separation was introduced by~\cite{isik2016single, 8045733}. ~\cite{isik2016single} introduced the deep unsupervised separation model. This method estimate the mask by extracting embedding to each segment of the spectrogram and clustering these. A deep attractor network that extract centroids in the high dimensional embedding spaces, in order to obtain the time-frequency bins for each speaker was presented in \cite{chen2017deep}.

%  In~\cite{wang2018alternative} multiple clustering network approaches were evaluated and a novel chimera network, which combines mask-inference networks with deep clustering networks, obtains an improvement of 0.7 dB on the WSJ0-2mix dataset over the alternative methods.

% Further works on speech separation include input with multiple channels (i.e. multiple microphones). In~\cite{markovich2009multichannel}, the authors present  an extension to the minimum variance distortionless response (MVDR) beamformer~\cite{capon1969high,frost1972algorithm}. The method includes the linearly constrained minimum variance (LCMV) beamformer~\cite{laufer2020global} which is designed to obtain the desired signals and to mitigate the interferences. The MVDR neural beamformer introduce in~\cite{xiao2016study}, predict a mask in time-frequency space, which is then used to estimate the MVDR beam, 
% showing an improvement over both the traditional MVDR method and delay-and-sum beamforming.

% The FaSNet (filter-and-sum network) method~\cite{luo2019fasnet} includes two-stage processing units. The first learns frame-level time-domain adaptive beamforming filters for a selected reference channel, and second stage calculates the filters for the remaining channels. 
% FaSNet improves the MVDR baseline results with $14.3\%$ relative word error rate reduction (RWERR). FaSNet was extended to form the transform-average-concatenate (TAC) model~\cite{luo2019end}. This method employs a transformation module that extract feature to each channel, a copy of these features undergoes global pooling. A concatenation module is then applied to the output of the first and the second modules. This method shows improvement in the separation for noisy environment, and experiments are conducted  with both a varying numbers of microphones and a fix geometry array configuration.
